Optimal Distributed Optimization on Slowly Time-Varying Graphs

We study optimal distributed first-order optimization algorithms when the network (i.e., communication constraints between the agents) changes with time. This problem is motivated by scenarios where agents experience network malfunctions. We provide a sufficient condition that guarantees a convergence rate with optimal (up lo logarithmic terms) dependencies on the network and function parameters if the network changes are constrained to a small percentage $\alpha$ of the total number of iterations. We call such networks slowly time-varying networks. Moreover, we show that Nesterov's method has an iteration complexity of $\Omega \big( \big(\sqrt{\kappa_\Phi \cdot \bar{\chi}} + \alpha \log(\kappa_\Phi \cdot \bar{\chi})\big) \log(1 / \varepsilon)\big)$ for decentralized algorithms, where $\kappa_\Phi$ is condition number of the objective function, and $\bar\chi$ is a worst case bound on the condition number of the sequence of communication graphs. Additionally, we provide an explicit upper bound on $\alpha$ in terms of the condition number of the objective function and network topologies.

==> figure_big1_2.tex <==
\begin{figure}[ht!]
	\centering
		\subfigure{\includegraphics[width=0.28\linewidth]{Figures/main-figure7}}
		\subfigure{\includegraphics[width=0.28\linewidth]{Figures/main-figure8}}
		\subfigure{\includegraphics[width=0.28\linewidth]{Figures/main-figure9}}
	\caption{A sequence of Erd\H{o}s-R\'enyi random graphs with $10$ nodes each changing every $50$ iterations.} 
\label{fig:changing1}
\end{figure}

==> figure_big2_2.tex <==
\begin{figure}[ht!]
	\centering
		\subfigure{\includegraphics[width=0.28\linewidth]{Figures/main-figure14}}
		\subfigure{\includegraphics[width=0.29\linewidth]{Figures/main-figure15}}
		\subfigure{\includegraphics[width=0.30\linewidth]{Figures/main-figure16}}
	\caption{Distance to Optimality and Distance to Consensus for a network of $100$ Agents on a sequence of graphs that shuffles between a complete graph and a path graph every (a,b) $50$ iterations, (c,d) $100$ iterations, and (e,f) $500$ iterations.}
\label{fig:cyle_star}
\end{figure}
